A 3D measurement workflow for assessing replication quality and tool degradation in moulded microfluidic channels

Mould-based replication, such as injection moulding with 3D-printed inserts, needs a check of how faithfully microchannels are transferred from master to polymer replica. It is usually limited to a width or depth ratio from one cross-section, which misses the sidewall shape and depends on where the section is taken. We present a workflow that assesses the whole channel from 3D scans of master and replica, without sectioning. The scans are registered on a common grid, and each height map is converted into a map of local slope. The correlation of the two slope maps over the channel interior, RQ$_d$, is reported with the channel dimensions and height- and slope-error maps. These outputs separate a change of shape from a change of size and locate it. A user can thereby compare mould materials, detect tool wear, and tell whether a deviation arose before or during moulding. On synthetic channels with known degradation, RQ$_d$ fell steadily as the sidewalls were rounded, whereas the height correlation levelled off. For injection moulding with stereolithography-printed inserts in three resins, RQ$_d$ ranged from 0.17 to 0.91 over fifteen insert-to-part pairs. The height correlation placed the ten well-formed channels within 0.03. Over a twenty-shot run, one insert's RQ$_d$ fell from 0.90 to 0.72 as its sidewalls wore, while its height correlation stayed above 0.93. We developed open-source software that implements the workflow. Because the workflow needs only registered 3D scans of a master and its replica, it can in principle be applied to other mould-based processes.

==> supplement_tables/s2_numbers.tex <==
\newcommand{\eqHT}{40}
\newcommand{\eqRTK}{52}
\newcommand{\eqW}{below the range}

